Online Job Failure Prediction in an HPC System

Modern High Performance Computing (HPC) systems are complex machines, with major impacts on economy and society. Along with their computational capability, their energy consumption is also steadily raising, representing a critical issue given the ongoing environmental and energetic crisis. Therefore, developing strategies to optimize HPC system management has paramount importance, both to guarantee top-tier performance and to improve energy efficiency. One strategy is to act at the workload level and highlight the jobs that are most likely to fail, prior to their execution on the system. Jobs failing during their execution unnecessarily occupy resources which could delay other jobs, adversely affecting the system performance and energy consumption. In this paper, we study job failure prediction at submit-time using classical machine learning algorithms. Our novelty lies in (i) the combination of these algorithms with Natural Language Processing (NLP) tools to represent jobs and (ii) the design of the approach to work in an online fashion in a real system. The study is based on a dataset extracted from a production machine hosted at the HPC centre CINECA in Italy. Experimental results show that our approach is promising.

==> chapters/backup.tex <==
% \subsection{D.A.V.I.D.E.}

% % DAVIDE was introduced in \cite{DAVIDE}
% % forse da rifrasare
% D.A.V.I.D.E.: (Development of an Added Value Infrastructure Designed in Europe)\cite{DAVIDE} is an energy aware ex-production HPC hosted at CINECA. 
% The cluster was deployed to production in 2017 (until 2020) and it entered the TOP500 and GREEN500 list in June of the same year. 
% The machine reach Petaflops performance and it based on OpenPOWER Architecture coupled with NVIDIA Tesla Pascal GPUs connected through NVLink switches.
% A more detailed description of the system's specifics is reported in Table.\ref{davide_sys_arch}.

% D.A.V.I.D.E. is endowed with ExaMon, which provides power consumption insights to the system through the collection of data from the main components (processors, memory, GPUs, fans) of the cluster.
% Moreover, it performs power capping of the machine at global and node level.


% \begin{table}[h!]
% \caption{D.A.V.I.D.E. system architecture.}\label{davide_sys_arch}
% \begin{center}
%     \begin{tabular}{|l|l|}
%     \hline
%     Specific &  Description\\
%     \hline
%     % Racks &  55\\
%     Architecture & OpenPower \\
%     Nodes & 45\\
%     Processors(per node) & 2 x OpenPower8 \\
%     Accelerators(per node) & 4 NVIDIA Tesla P100 SXM2 \\
%     Peak Performance &  1 PFlop/s\\
%     Internal Network & 2xIB EDR, 2x1GbE\\
%     \hline
%     \end{tabular}
%     \end{center}
% \end{table}

% Alike Marconi100, also D.A.V.I.D.E. relies on SLURM as a DRMS, making its workload comparable to the one of Marconi100.

% \begin{minipage}{0.49\textwidth}

% \caption{Job ECs distribution.}\label{labels_dist_m100}
% \begin{center}
%     \begin{tabular}{|l|l|l|}
%     \hline
%     \textbf{Code} &  \textbf{Number} & \textbf{Percentage} \\
%     \hline
%     0 & 924252 & 89\% \\
%     1 & 93180 & 9\% \\
%     2 & 2385 & 0.2\% \\
%     43 & 1082 & 0.1\%\\ 
%     127 & 3562 & 0.3\%\\ 
%     134 & 2948 & 0.3\%\\ 
%     139 & 3381 & 0.2\%\\ 
%     \hline
%     Other & 6489 & 0.6\%\\
%     \hline
%     \end{tabular}
%     \end{center}

% \end{minipage}
% \end{table}


% \subsection{Data Extraction Tool}

% %DA RIFRASARE
% \zk{I suggest to remove this subsection entirely: The collection of the metrics and the monitoring of the system is handled through ExaMon\footnote{https://github.com/EEESlab/examon}.
% ExaMon is an holistic open-source framework \cite{10.5555/3130379.3130626} for performance and energy monitoring of large-scale distributed architectures.
% The framework relies on high-scalable and distributed SW, which gather data from both HW sensors and SW plugins to provide real-time insights about the state of the facilities.
% Hardware sensors collect several metrics about the usage and the state of the resources, such as CPU load of all the cores in the supercomputer nodes, CPU clock, instructions per second, memory accesses (bytes written and read), fan speed, the temperature of the room hosting the system racks, power consumption (at different levels), etc.
% SW-based plugins, on the other hand, gather the information provided by the resource manager, consisting of the job request (e.g., job id, job name, job user, job partition/queue), the requested resources(number of requested nodes, requested cores, requested GPUs, etc.), and the resources actually used.}
% % All the information collected by ExaMon are then saved in an instance of Apache Cassandra\footnote{https://cassandra.apache.org/}, a NoSQL database (DB) optimized to work in distributed architectures.
% % The DB is equipped with a KairosDB\footnote{https://github.com/kairosdb/kairosdb} instance, to handle time-series data more efficiently.
% % All of the ExaMon's layers communicate with each other through the MQTT protocol\footnote{https://mqtt.org}, a lightweight messaging protocol for the Internet of Things (IoT). 


% \begin{figure}[h]
% \begin{center}
% \begin{minipage}{0.49\textwidth}

% \includegraphics[width=\textwidth]{figures/states_distributionpng.png}
% \centering
% a)
% \end{minipage}
% \begin{minipage}{0.49\textwidth}

% \includegraphics[width=\textwidth]{figures/states_distrib_weekday.png}
% \centering
% b)
% \end{minipage}
% \begin{minipage}{0.75\textwidth}

% \includegraphics[width=\textwidth]{figures/stats_distrib_hour.png}
% \centering
% c)
% \end{minipage}
% \end{center}
% \caption{The distribution of the exit state labels from May 2020 to October 2020, divided by a) month, b) weekday and c) hour of the day.} \label{figdistmonth}
% \end{figure}

% \begin{minipage}{0.49\textwidth}
% \begin{center}
%     \begin{tabular}{|l|l|}
%     \hline
%     \textbf{EC}  & \textbf{\%} \\
%     \hline
%     0 &  89\% \\
%     1 &  9\% \\
%     2 &  0.2\% \\
%     43 & 0.1\%\\ 
%     127 & 0.3\%\\ 
%     134 & 0.3\%\\ 
%     139 & 0.2\%\\ 
%     \hline
%     Other & 0.6\%\\
%     \hline
%     \end{tabular}
%     \end{center}
% \caption{Job EC distribution in the considered subset of the M100 dataset.}\label{labels_dist_m100}
% \end{minipage}

% \begin{table}[h!]
% \caption{Models results on a) completed and b) failed classes in the online setting.}
% \label{results_classes}
% \begin{center}
% \begin{minipage}{0.49\textwidth}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|l|l|l|l|}
    
%     \hline
%     Model &  &  &  \\
%     (Encoding + Classification) &  F1 & Precision & Recall \\
%     \hline
%     INT+DT & 0.80 & 0.84 & 0.79 \\
%     INT+LR & 0.85 & 0.79 & \textbf{0.95}\\
%     INT+RF & 0.85 & 0.84 & 0.88 \\
%     SB+DT & 0.80 & 0.84 & 0.78 \\
%     SB+LR & 0.85 & 0.82 & 0.89 \\
%     SB+RF & \textbf{0.87} & 0.83 & 0.92  \\
%     \hline
%     INT+CD & 0.84 & 0.86 & 0.82 \\
%     % INT+ED & 0.84 & 0.86 & 0.83 \\
%     INT+MWD & 0.84 & \textbf{0.87} & 0.83 \\
    
    
    
%     SB+CD & 0.84 & \textbf{0.87} & 0.83 \\
    
%     SB+ED & 0.84 & \textbf{0.87} & 0.83 \\
    
%     SB+MWD & 0.85 & \textbf{0.87} & 0.83 \\

%     \hline
%     MAJORITY & \textbf{0.87} & 0.79 & 1\\
%     RANDOM & 0.61 & 0.79 & 0.5 \\
%     \hline
%     \end{tabular} }
%     \centering
% a)
% \end{minipage}   
%     \hfill
% \begin{minipage}{0.49\textwidth}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|l|l|l|l|}
%     % \caption{Models results on completed class.}
%     \hline
%      Model &  &  &  \\
%     (Encoding + Classification) &  F1 & Precision & Recall \\
%     \hline
%     INT+DT & 0.41 & 0.44 & 0.46 \\
%     INT+LR & 0.06 & 0.26 & 0.06\\
%     INT+RF & 0.43 & 0.55 & 0.41 \\
%     SB+DT & 0.41 & 0.39 & 0.47 \\
%     SB+LR & 0.34 & 0.50 & 0.30 \\
%     SB+RF & 0.40 & \textbf{0.58} & 0.34  \\
%     \hline
%     INT+CD & 0.52 & 0.52 & 0.56 \\
%     INT+ED & 0.51 & 0.51 & 0.55 \\
%     INT+MWD & 0.52 & 0.51 & 0.55 \\
    
    
    
%     SB+CD & \textbf{0.54} & 0.54 & \textbf{0.59} \\
    
%     SB+ED & \textbf{0.54} & 0.53 & \textbf{0.59} \\
    
%     SB+MWD & \textbf{0.54} & 0.54 & \textbf{0.59} \\
    
%     \hline
%     MAJORITY & 0 & 0 & 0\\
%     RANDOM & 0.28 & 0.21 & 0.5 \\
%     \hline
%     \end{tabular}}
%     \centering
% b)
% \end{minipage}
%     \end{center}
% \end{table}

% \begin{tabular}{|l|l|}
%     \hline
%     \textbf{Name} &  \textbf{\%}\\
%     \hline
%     Completed & 83.2\% \\
%     Failed & 9.6\% \\
%     Cancelled & 5.4\%\\
%     Timeout & 1.4\% \\
%     Out of memory & 0.4\%\\
%     Preempted & 0 \\
%     Node fail & 0.02\% \\
%     \hline
%     \end{tabular}

% \begin{table}[h!]

% \begin{center}
    
%     \begin{tabular}{|l|l|l|l||l|l|l||l|l|l|}
%     \hline
%     Model & T F1-M & T Prec-M & T Rec-M & C F1 & C Prec & C Rec & F F1 & F Prec & F Rec\\
     
%     \hline
%     Supervised  & & & & & & & & & \\
%     INT+DT & \textbf{0.90} & \textbf{0.90} & \textbf{0.90} & \textbf{0.98} & \textbf{0.98} & 0.98 & \textbf{0.82} & 0.82 & \textbf{0.82}\\
%     INT+LR & 0.48 & 0.51 & 0.50 & 0.94 & 0.88 & 0.99 & 0.02 & 0.14 & 0.01\\
%     INT+RF & \textbf{0.90} & \textbf{0.90} & \textbf{0.90} & \textbf{0.98} & \textbf{0.98} & 0.98 & \textbf{0.82} & \textbf{0.83} & \textbf{0.82} \\
%     SB+DT &  0.83 & 0.83 & 0.83 & 0.96 & 0.96 & 0.96 & 0.70 & 0.69 & 0.70 \\
%     SB+LR & 0.70 & 0.79 & 0.67 & 0.95 & 0.92 & 0.98 &  0.46 & 0.66 & 0.36 \\
%     SB+RF & 0.87 & 0.89 & 0.85 & 0.97 & 0.96 & 0.98 & 0.76 & 0.82  & 0.72\\
%     \hline
%     Unsupervised  & & & & & & & & & \\
%     INT+CD & 0.89 & \textbf{0.90} & 0.88 & \textbf{0.98} & 0.97 & 0.98 & 0.80 & \textbf{0.83} & 0.78\\
%     % INT+ED & \textbf{0.96} & 0.89 & \textbf{0.90} & 0.88 \\
%     INT+MWD & 0.89 & \textbf{0.90} & 0.88 & \textbf{0.98} & 0.97 & 0.98 & 0.83 & 0.78 & 0.81\\

%     SB+CD &  0.86 & 0.87 & 0.85 & 0.97 & 0.97 & 0.97 & 0.75 & 0.78 & 0.73\\
    
%     % SB+ED & 0.94 & 0.86 & 0.87 & 0.85  \\
    
%     SB+MWD & 0.86 & 0.87 & 0.85 & 0.97 & 0.96 & 0.97 & 0.75 & 0.78 & 0.73 \\
    
%     \hline
%     Random  & & & & & & & & & \\
%     Majority & 0.47 & 0.44 & 0.50 & 0.94 & 0.88 & \textbf{1.00} & 0.00 & 0.00 & 0.00 \\
%     Random  & 0.41 & 0.50 & 0.50 & 0.64 & 0.88 & 0.50 & 0.19 & 0.11 & 0.50  \\
%     \hline
%     \end{tabular}
%     \end{center}
%     \caption{Results of the model on the offline random settings, divided in Total (T), Completed class (C) and Failed class (F). For the total task we consider the macro average metrics (M) f1, precision and recall. The model name comprises encoding+classification method.}\label{results_global_split}
% \end{table}

==> chapters/data.tex <==
The first dataset is derived from Marconi100 workload (M100)\cite{andrea_borghesi_2023_m100}.
% descrivi m100, e di che hai preso solo il primo anno perchè ci sono gli exit code.




Insights sui dati, distribuzione, grafici vari e studio di anomalie ecc
